Long-term Stellar Variability in the Galactic Centre Region

We report the detection of variable stars within a 11.5' x 11.5' region near the Galactic centre (GC) that includes the Arches and Quintuplet clusters, as revealed by the VISTA Variables in the Via Lactea (VVV) survey. There are 353 sources that show Ks-band variability, of which the large majority (81%) correspond to red giant stars, mostly in the asymptotic giant branch (AGB) phase. We analyze a population of 52 red giants with long-term trends that cannot be classified into the typical pulsating star categories. Distances and extinctions are calculated for 9 Mira variables, and we discuss the impact of the chosen extinction law on the derived distances. We also report the presence of 48 new identified young stellar object (YSO) candidates in the region.

==> Table1_full_version.tex <==
\section{The full version of Table~1.}

\newpage
\begin{landscape}
	\begin{table}
	\caption{Summary with the main properties of the variable stars found.}
    \label{tbl:tbl-1}
    \begin{tabular}{lcccccccccccccccc}
    \hline
    Name & RA & Dec. & $l$ & $b$ & $J$ & $H$ & $K_S$ & $[3.6]$ & $[4.5]$ & $[5.8]$ & $[8.0]$ & $\langle K_S \rangle$ & $\Delta K_S$ & Period & Class & Lit. ref.$^a$ \\
 & (J2000) & (J2000) & (\degree) & (\degree) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (mag) & (days) & & \\
	\hline
NV001 & 17:45:21.16 & -28:50:48.36 & 0.045810 & 0.096523 & -99.9 & 18.13 & 14.25 & -99.9 & -99.9 & -99.9 & -99.9 & 14.16 & 0.97 & 1248 & SR & -99.9 \\
NV002 & 17:45:23.25 & -28:50:58.59 & 0.047359 & 0.088541 & 19.03 & 14.55 & 12.03 & 10.52 & 10.1 & 9.68 & 8.99 & 12.23 & 0.4 & -99.9 & IRR & -99.9 \\
NV003 & 17:45:23.46 & -28:50:06.46 & 0.060115 & 0.095437 & -99.9 & 18.44 & 14.76 & -99.9 & 11.62 & 11.45 & -99.9 & 14.54 & 1.11 & 1144 & SR & -99.9 \\
NV004 & 17:45:27.15 & -28:50:17.78 & 0.064462 & 0.082291 & -99.9 & -99.9 & 16.39 & -99.9 & -99.9 & -99.9 & -99.9 & 16.19 & 1.29 & -99.9 & Eruptive & -99.9 \\
NV005 & 17:45:28.11 & -28:49:34.76 & 0.076481 & 0.085539 & -99.9 & 17.15 & 12.28 & 8.9 & 8.14 & -99.9 & -99.9 & 12.0 & 1.06 & 498 & Mira & 1 \\
NV006 & 17:45:30.82 & -28:51:06.02 & 0.060007 & 0.063877 & -99.9 & 17.45 & 13.37 & -99.9 & -99.9 & -99.9 & -99.9 & 13.73 & 1.24 & -99.9 & LPV & -99.9 \\
NV007 & 17:45:32.07 & -28:48:40.54 & 0.096883 & 0.081029 & -99.9 & 14.68 & 11.97 & 10.35 & 10.01 & -99.9 & 9.67 & 12.02 & 0.46 & -99.9 & IRR & -99.9 \\
NV008 & 17:45:32.66 & -28:52:07.61 & 0.048898 & 0.049242 & -99.9 & 16.21 & 13.23 & -99.9 & 10.97 & 10.29 & -99.9 & 13.44 & 0.84 & 1502 & SR & -99.9 \\
NV009 & 17:45:33.19 & -28:52:23.69 & 0.046093 & 0.045266 & -99.9 & 15.99 & 13.07 & 10.96 & 10.45 & 9.49 & -99.9 & 13.34 & 0.51 & -99.9 & LPV & -99.9 \\
NV010 & 17:45:33.75 & -28:48:36.44 & 0.101040 & 0.076409 & -99.9 & 15.75 & 13.48 & 12.52 & 12.52 & -99.9 & -99.9 & 13.6 & 0.5 & -99.9 & LPV & -99.9 \\
NV011 & 17:45:34.53 & -28:47:34.48 & 0.117224 & 0.082929 & -99.9 & 16.89 & 12.29 & 10.97 & 9.51 & 9.05 & -99.9 & 12.8 & 1.03 & -99.9 & IRR & -99.9 \\
NV012 & 17:45:34.57 & -28:52:11.92 & 0.051510 & 0.042669 & -99.9 & 15.68 & 12.48 & 10.57 & 10.13 & 9.2 & -99.9 & 12.46 & 0.42 & 1738 & SR & -99.9 \\
NV013 & 17:45:35.65 & -28:47:43.67 & 0.117173 & 0.078115 & -99.9 & 16.05 & 13.54 & 12.18 & 11.6 & -99.9 & -99.9 & 13.62 & 0.47 & -99.9 & LPV & -99.9 \\
NV014 & 17:45:35.67 & -28:51:51.48 & 0.058450 & 0.042200 & -99.9 & 15.06 & 12.24 & -99.9 & -99.9 & -99.9 & -99.9 & 12.31 & 0.48 & 1430 & SR & -99.9 \\
NV015 & 17:45:36.19 & -28:52:34.46 & 0.049252 & 0.034350 & -99.9 & 18.0 & 14.86 & -99.9 & -99.9 & -99.9 & -99.9 & 15.35 & 1.22 & -99.9 & IRR & -99.9 \\
NV016 & 17:45:36.52 & -28:52:36.19 & 0.049477 & 0.033063 & -99.9 & 15.82 & 12.21 & 10.66 & 9.83 & 9.47 & -99.9 & 12.59 & 0.75 & -99.9 & IRR & -99.9 \\
NV017 & 17:45:36.85 & -28:52:31.56 & 0.051192 & 0.032721 & -99.9 & 15.37 & 11.90 & 10.06 & 9.46 & 8.21 & -99.9 & 11.88 & 0.46 & 1003 & SR & -99.9 \\
NV018 & 17:45:36.93 & -28:52:56.19 & 0.045514 & 0.028888 & -99.9 & -99.9 & 13.91 & 12.82 & 11.1 & -99.9 & -99.9 & 14.88 & 3.47 & -99.9 & RCB? & -99.9 \\
NV019 & 17:45:37.16 & -28:52:37.58 & 0.050355 & 0.030883 & -99.9 & 18.06 & 14.65 & -99.9 & -99.9 & -99.9 & -99.9 & 14.86 & 0.86 & -99.9 & Dipper & -99.9 \\
NV020 & 17:45:37.25 & -28:52:51.92 & 0.047123 & 0.028530 & -99.9 & 15.72 & 11.74 & 10.47 & 9.21 & 8.25 & 7.44 & 11.9 & 0.81 & -99.9 & IRR & -99.9 \\
NV021 & 17:45:37.27 & -28:52:59.88 & 0.045281 & 0.027304 & -99.9 & -99.9 & 16.68 & -99.9 & -99.9 & -99.9 & -99.9 & 15.19 & 1.47 & -99.9 & Eruptive & -99.9 \\
NV022 & 17:45:37.30 & -28:52:38.45 & 0.050428 & 0.030301 & -99.9 & -99.9 & 16.07 & -99.9 & -99.9 & -99.9 & -99.9 & 15.12 & 0.98 & -99.9 & Dipper & -99.9 \\
NV023 & 17:45:37.36 & -28:50:21.42 & 0.083019 & 0.049961 & -99.9 & 16.43 & 13.15 & -99.9 & -99.9 & -99.9 & -99.9 & 13.01 & 0.38 & 259 & SR & -99.9 \\
NV024 & 17:45:37.50 & -28:46:55.46 & 0.132114 & 0.079342 & -99.9 & 15.16 & 12.57 & 11.42 & 11.04 & 10.01 & -99.9 & 12.73 & 0.61 & -99.9 & LPV & -99.9 \\
NV025 & 17:45:37.54 & -28:50:44.99 & 0.077767 & 0.046002 & -99.9 & 17.20 & 13.52 & -99.9 & 11.06 & 10.61 & -99.9 & 13.32 & 0.44 & -99.9 & IRR & -99.9 \\
NV026 & 17:45:38.05 & -28:52:27.59 & 0.054412 & 0.029561 & -99.9 & 17.68 & 14.22 & -99.9 & -99.9 & -99.9 & -99.9 & 14.02 & 0.87 & -99.9 & LPV & -99.9 \\
NV027 & 17:45:38.53 & -28:52:19.61 & 0.057222 & 0.029214 & -99.9 & 18.07 & 15.22 & -99.9 & -99.9 & -99.9 & -99.9 & 15.51 & 0.94 & -99.9 & Dipper & -99.9 \\
NV028 & 17:45:38.60 & -28:50:43.11 & 0.080243 & 0.042948 & -99.9 & 16.51 & 12.36 & 11.16 & 9.83 & 9.43 & -99.9 & 12.21 & 0.48 & -99.9 & LPV & -99.9 \\
NV029 & 17:45:38.65 & -28:52:50.89 & 0.050035 & 0.024310 & -99.9 & -99.9 & 14.18 & -99.9 & 11.35 & -99.9 & -99.9 & 14.61 & 1.03 & -99.9 & LPV & -99.9 \\
NV030 & 17:45:38.97 & -28:52:41.55 & 0.052849 & 0.024677 & -99.9 & 15.71 & 12.37 & 10.85 & -99.9 & -99.9 & -99.9 & 12.92 & 1.0 & 1382 & SR & -99.9 \\
NV031 & 17:45:38.99 & -28:52:25.70 & 0.056656 & 0.026893 & -99.9 & 17.45 & 13.71 & 13.08 & 11.54 & -99.9 & -99.9 & 13.78 & 1.17 & -99.9 & IRR & -99.9 \\
NV032 & 17:45:39.09 & -28:52:45.14 & 0.052229 & 0.023779 & -99.9 & 17.04 & 12.30 & 9.96 & 8.32 & 7.72 & 7.52 & 12.15 & 1.09 & -99.9 & IRR & 1 \\
NV033 & 17:45:40.16 & -28:46:51.91 & 0.138030 & 0.071543 & 18.18 & 14.81 & 12.48 & 10.14 & 9.35 & 8.76 & -99.9 & 12.51 & 0.6 & 311 & SR & -99.9 \\
NV034 & 17:45:40.21 & -28:52:53.49 & 0.052388 & 0.019067 & -99.9 & 16.51 & 12.95 & -99.9 & -99.9 & -99.9 & -99.9 & 12.84 & 0.24 & -99.9 & IRR & -99.9 \\
NV035 & 17:45:40.70 & -28:45:27.64 & 0.159028 & 0.082069 & -99.9 & -99.9 & 16.09 & -99.9 & 12.65 & -99.9 & -99.9 & 15.54 & 1.79 & -99.9 & Eruptive/FUor & -99.9 \\
NV036 & 17:45:40.74 & -28:52:36.65 & 0.057376 & 0.019874 & 17.71 & 14.82 & 13.13 & -99.9 & -99.9 & -99.9 & -99.9 & 13.16 & 0.45 & 0.5564 & EB & 2 \\
NV037 & 17:45:40.85 & -28:49:14.67 & 0.105486 & 0.048742 & -99.9 & 18.08 & 15.77 & -99.9 & -99.9 & -99.9 & -99.9 & 15.65 & 1.48 & -99.9 & Eruptive/EXor & -99.9 \\
NV038 & 17:45:41.06 & -28:44:22.79 & 0.175093 & 0.090326 & -99.9 & 17.25 & 15.31 & -99.9 & -99.9 & -99.9 & -99.9 & 15.54 & 1.06 & -99.9 & Fader & -99.9 \\
NV039 & 17:45:41.07 & -28:52:51.98 & 0.054384 & 0.016604 & -99.9 & 16.32 & 12.45 & 9.93 & 9.18 & 8.75 & -99.9 & 12.66 & 0.48 & -99.9 & IRR & -99.9 \\
NV040 & 17:45:41.62 & -28:45:04.70 & 0.166226 & 0.082507 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & 16.11 & 1.01 & -99.9 & Eruptive & -99.9 \\
NV041 & 17:45:41.76 & -28:45:25.70 & 0.161507 & 0.079044 & -99.9 & 16.62 & 13.58 & 12.27 & -99.9 & 10.95 & -99.9 & 13.5 & 0.83 & -99.9 & IRR & -99.9 \\
NV042 & 17:45:41.86 & -28:45:18.62 & 0.163373 & 0.079761 & -99.9 & 16.81 & 14.02 & -99.9 & -99.9 & -99.9 & -99.9 & 14.45 & 1.03 & -99.9 & LPV & -99.9 \\
NV043 & 17:45:41.91 & -28:45:26.19 & 0.161681 & 0.078497 & -99.9 & 16.70 & 13.06 & -99.9 & 11.05 & -99.9 & -99.9 & 13.88 & 1.35 & -99.9 & LPV & -99.9 \\
NV044 & 17:45:41.93 & -28:52:45.48 & 0.057544 & 0.014890 & -99.9 & 15.72 & 13.21 & -99.9 & -99.9 & -99.9 & -99.9 & 13.57 & 1.53 & -99.9 & LPV & -99.9 \\
NV045 & 17:45:42.31 & -28:46:07.44 & 0.152659 & 0.071281 & 18.61 & 14.16 & 11.81 & 10.48 & 10.25 & 9.67 & 9.02 & 11.87 & 0.26 & -99.9 & IRR & -99.9 \\
NV046 & 17:45:42.40 & -28:45:15.22 & 0.165210 & 0.078560 & -99.9 & 17.36 & 13.83 & 12.77 & 11.98 & -99.9 & -99.9 & 13.64 & 0.82 & 428 & SR & -99.9 \\
NV047 & 17:45:42.49 & -28:45:41.57 & 0.159140 & 0.074458 & 18.96 & 15.42 & 13.31 & -99.9 & -99.9 & -99.9 & -99.9 & 13.88 & 0.89 & -99.9 & LPV & -99.9 \\
NV048 & 17:45:42.80 & -28:45:13.98 & 0.166268 & 0.077492 & -99.9 & 17.93 & 14.38 & 12.57 & 11.53 & 10.41 & -99.9 & 14.38 & 1.67 & -99.9 & LPV & -99.9 \\
NV049 & 17:45:42.94 & -28:47:20.25 & 0.136593 & 0.058786 & -99.9 & 17.69 & 14.48 & -99.9 & -99.9 & -99.9 & -99.9 & 14.84 & 1.0 & -99.9 & LPV & -99.9 \\
NV050 & 17:45:43.83 & -28:45:18.51 & 0.167154 & 0.073620 & -99.9 & 17.80 & 15.49 & -99.9 & -99.9 & -99.9 & -99.9 & 15.81 & 1.3 & -99.9 & Dipper & -99.9 \\
NV051 & 17:45:43.93 & -28:43:49.87 & 0.188351 & 0.086152 & -99.9 & 16.18 & 13.72 & 11.8 & 11.36 & 11.03 & -99.9 & 13.76 & 0.95 & -99.9 & IRR & -99.9 \\
NV052 & 17:45:43.98 & -28:45:41.26 & 0.162036 & 0.069877 & -99.9 & -99.9 & 11.98 & -99.9 & -99.9 & -99.9 & -99.9 & 13.59 & 3.75 & -99.9 & RCB? & -99.9 \\
NV053 & 17:45:43.98 & -28:51:57.84 & 0.072744 & 0.015388 & -99.9 & 14.43 & 11.70 & -99.9 & -99.9 & -99.9 & -99.9 & 11.6 & 0.24 & -99.9 & IRR & 1 \\
NV054 & 17:45:44.17 & -28:47:15.18 & 0.140125 & 0.055698 & -99.9 & 14.71 & 11.95 & 10.55 & 10.05 & 9.51 & -99.9 & 12.01 & 0.7 & -99.9 & IRR & 1 \\
NV055 & 17:45:44.19 & -28:43:46.12 & 0.189748 & 0.085866 & -99.9 & 17.77 & 15.12 & -99.9 & -99.9 & -99.9 & -99.9 & 15.57 & 1.16 & 749 & SR & -99.9 \\
NV056 & 17:45:44.33 & -28:47:12.76 & 0.141006 & 0.055546 & 18.37 & 14.57 & 12.46 & 11.45 & 11.25 & -99.9 & -99.9 & 12.66 & 0.5 & 1492 & SR & -99.9 \\
NV057 & 17:45:44.43 & -28:45:39.42 & 0.163332 & 0.068732 & -99.9 & -99.9 & 15.49 & -99.9 & -99.9 & -99.9 & -99.9 & 15.38 & 1.2 & -99.9 & Dipper & -99.9 \\
NV058 & 17:45:44.47 & -28:45:09.48 & 0.170500 & 0.072951 & -99.9 & 15.52 & 13.20 & -99.9 & -99.9 & -99.9 & -99.9 & 12.57 & 0.76 & -99.9 & LPV & 1 \\
NV059 & 17:45:44.95 & -28:47:44.97 & 0.134554 & 0.048938 & -99.9 & 16.91 & 13.65 & 11.87 & 11.15 & 9.69 & -99.9 & 13.87 & 0.53 & -99.9 & IRR & -99.9 \\
NV060 & 17:45:45.29 & -28:47:56.13 & 0.132544 & 0.046283 & -99.9 & 17.59 & 15.28 & -99.9 & -99.9 & -99.9 & -99.9 & 15.78 & 1.22 & -99.9 & Dipper & -99.9 \\
NV061 & 17:45:45.35 & -28:47:07.30 & 0.144236 & 0.053161 & 17.79 & 14.59 & 12.80 & 11.62 & 11.43 & -99.9 & -99.9 & 12.9 & 0.37 & -99.9 & IRR & -99.9 \\
NV062 & 17:45:45.35 & -28:47:37.61 & 0.137058 & 0.048765 & -99.9 & 14.83 & 11.61 & 11.07 & 10.09 & 9.52 & -99.9 & 12.04 & 0.94 & -99.9 & LPV & 1 \\
NV063 & 17:45:45.53 & -28:47:56.16 & 0.133003 & 0.045513 & 19.09 & 14.21 & 11.71 & 10.32 & 10.02 & 9.62 & -99.9 & 11.81 & 0.61 & -99.9 & IRR & 1 \\
NV064 & 17:45:45.63 & -28:48:20.59 & 0.127402 & 0.041665 & -99.9 & 14.50 & 11.49 & 9.6 & 9.15 & 8.75 & -99.9 & 11.38 & 0.4 & 385 & SR & -99.9 \\
NV065 & 17:45:45.74 & -28:51:30.32 & 0.082611 & 0.013888 & -99.9 & 16.94 & 13.64 & 11.44 & 11.04 & -99.9 & -99.9 & 13.57 & 0.94 & -99.9 & LPV & -99.9 \\
NV066 & 17:45:45.75 & -28:47:37.82 & 0.137757 & 0.047502 & -99.9 & 14.70 & 11.71 & 10.64 & -99.9 & 9.41 & -99.9 & 11.72 & 0.36 & -99.9 & IRR & 1 \\
NV067 & 17:45:46.32 & -28:45:51.08 & 0.164171 & 0.061141 & -99.9 & 14.25 & 11.60 & 10.03 & 9.81 & 8.7 & 7.82 & 11.85 & 1.01 & -99.9 & IRR & -99.9 \\
NV068 & 17:45:46.48 & -28:51:32.70 & 0.083460 & 0.011230 & -99.9 & 15.27 & 12.03 & 11.02 & 10.32 & 9.12 & -99.9 & 11.77 & 0.29 & 443 & SR & -99.9 \\
NV069 & 17:45:46.55 & -28:52:13.01 & 0.074032 & 0.005182 & -99.9 & 17.90 & 14.80 & -99.9 & -99.9 & -99.9 & -99.9 & 14.67 & 1.08 & -99.9 & RCB? & -99.9 \\
NV070 & 17:45:47.15 & -28:45:35.42 & 0.169464 & 0.060816 & -99.9 & 17.03 & 13.53 & 12.16 & 11.18 & -99.9 & -99.9 & 14.23 & 1.25 & 926 & SR & -99.9 \\
NV071 & 17:45:47.40 & -28:51:40.35 & 0.083397 & 0.007249 & -99.9 & 14.87 & 12.35 & 11.14 & 10.98 & 11.68 & -99.9 & 12.37 & 0.42 & -99.9 & IRR & -99.9 \\
NV072 & 17:45:47.65 & -28:47:33.38 & 0.142442 & 0.042192 & -99.9 & -99.9 & 15.17 & 13.01 & 12.35 & -99.9 & -99.9 & 15.37 & 1.02 & -99.9 & Dipper & -99.9 \\
NV073 & 17:45:47.86 & -28:47:22.22 & 0.145485 & 0.043155 & -99.9 & 17.73 & 15.50 & -99.9 & -99.9 & -99.9 & -99.9 & 15.74 & 1.52 & -99.9 & Fader/Dipper & -99.9 \\
NV074 & 17:45:47.92 & -28:51:09.30 & 0.091743 & 0.010129 & -99.9 & 16.48 & 13.04 & 10.54 & 10.05 & -99.9 & -99.9 & 13.56 & 1.14 & 598 & SR & -99.9 \\
NV075 & 17:45:48.14 & -28:48:43.96 & 0.126637 & 0.030455 & -99.9 & 16.01 & 13.02 & 11.24 & 10.92 & 10.11 & -99.9 & 13.61 & 1.58 & -99.9 & IRR & 1 \\
NV076 & 17:45:48.16 & -28:52:25.59 & 0.074109 & -0.00165 & -99.9 & 17.13 & 13.31 & -99.9 & -99.9 & -99.9 & -99.9 & 13.52 & 0.6 & -99.9 & IRR & 1 \\
NV077 & 17:45:48.39 & -28:47:47.91 & 0.140390 & 0.037805 & -99.9 & 15.20 & 12.79 & 12.4 & -99.9 & -99.9 & -99.9 & 13.07 & 0.87 & -99.9 & IRR & -99.9 \\
NV078 & 17:45:48.45 & -28:49:18.14 & 0.119104 & 0.024573 & -99.9 & 16.22 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & 13.42 & 1.17 & -99.9 & LPV & -99.9 \\
NV079 & 17:45:48.58 & -28:47:30.46 & 0.144886 & 0.039742 & -99.9 & 15.99 & 13.41 & -99.9 & -99.9 & -99.9 & -99.9 & 13.58 & 0.86 & -99.9 & IRR & -99.9 \\
NV080 & 17:45:48.71 & -28:47:33.69 & 0.144375 & 0.038857 & -99.9 & 15.86 & 12.65 & -99.9 & 10.44 & -99.9 & -99.9 & 12.36 & 0.55 & -99.9 & LPV & -99.9 \\
NV081 & 17:45:49.09 & -28:52:03.62 & 0.081085 & -0.00137 & -99.9 & 16.20 & 12.51 & -99.9 & -99.9 & 9.43 & -99.9 & 12.59 & 1.2 & 1556 & SR & -99.9 \\
NV082 & 17:45:49.12 & -28:47:50.96 & 0.141065 & 0.035072 & -99.9 & 17.95 & 14.36 & -99.9 & -99.9 & -99.9 & -99.9 & 14.71 & 0.9 & -99.9 & LPV & -99.9 \\
NV083 & 17:45:49.62 & -28:48:02.43 & 0.139297 & 0.031851 & -99.9 & 14.73 & 12.19 & 11.09 & 10.69 & 10.08 & -99.9 & 12.34 & 0.66 & -99.9 & IRR & -99.9 \\
NV084 & 17:45:49.67 & -28:48:21.64 & 0.134822 & 0.028942 & -99.9 & 15.27 & 12.48 & 11.19 & 10.73 & -99.9 & -99.9 & 12.56 & 0.31 & -99.9 & IRR & -99.9 \\
NV085 & 17:45:49.76 & -28:51:12.56 & 0.094474 & 0.003915 & -99.9 & 17.40 & 13.88 & 10.73 & 9.87 & 8.95 & -99.9 & 13.97 & 1.02 & -99.9 & LPV & -99.9 \\
NV086 & 17:45:49.88 & -28:47:45.23 & 0.143866 & 0.033534 & -99.9 & 18.10 & 15.34 & -99.9 & -99.9 & -99.9 & -99.9 & 15.45 & 1.16 & -99.9 & Dipper & -99.9 \\
NV087 & 17:45:50.03 & -28:43:46.67 & 0.200735 & 0.067559 & 18.91 & 16.24 & 13.69 & 13.07 & 12.13 & -99.9 & -99.9 & 13.98 & 1.96 & -99.9 & RCB/DYPer? & -99.9 \\
NV088 & 17:45:50.06 & -28:49:47.06 & 0.115305 & 0.015371 & -99.9 & -99.9 & 13.84 & 12.01 & 11.06 & 10.19 & -99.9 & 13.92 & 0.66 & -99.9 & LPV & -99.9 \\
NV089 & 17:45:50.08 & -28:43:38.96 & 0.202655 & 0.068521 & -99.9 & 18.02 & 15.39 & -99.9 & -99.9 & -99.9 & -99.9 & 15.23 & 1.8 & -99.9 & Eruptive/EXor & -99.9 \\
NV090 & 17:45:50.09 & -28:43:49.07 & 0.200278 & 0.067027 & -99.9 & 17.90 & 15.40 & -99.9 & -99.9 & -99.9 & -99.9 & 15.73 & 1.25 & -99.9 & Dipper & -99.9 \\
NV091 & 17:45:50.15 & -28:43:40.72 & 0.202357 & 0.068074 & 16.31 & 14.56 & 12.47 & 11.45 & 11.24 & 10.54 & -99.9 & 12.48 & 0.38 & -99.9 & IRR & -99.9 \\
NV092 & 17:45:50.15 & -28:52:18.74 & 0.079518 & -0.00687 & -99.9 & 17.29 & 12.92 & 9.82 & 9.33 & 8.66 & 8.38 & 12.35 & 0.6 & -99.9 & IRR & 1 \\
NV093 & 17:45:50.17 & -28:47:22.65 & 0.149771 & 0.035898 & -99.9 & 17.55 & 14.70 & -99.9 & -99.9 & -99.9 & -99.9 & 14.84 & 0.84 & -99.9 & LPV & -99.9 \\
NV094 & 17:45:50.23 & -28:52:30.24 & 0.076935 & -0.00876 & 18.97 & 14.49 & 12.02 & 10.74 & 10.56 & 9.68 & -99.9 & 12.1 & 0.29 & -99.9 & LPV & -99.9 \\
NV095 & 17:45:50.28 & -28:48:44.54 & 0.130554 & 0.023724 & -99.9 & 16.66 & 12.87 & 11.59 & 10.65 & -99.9 & -99.9 & 12.97 & 0.36 & -99.9 & IRR & -99.9 \\
NV096 & 17:45:50.55 & -28:43:56.82 & 0.199302 & 0.064490 & -99.9 & 15.61 & 12.31 & 10.83 & 10.38 & 9.72 & -99.9 & 12.58 & 0.98 & 470 & SR & 1 \\
NV097 & 17:45:50.66 & -28:43:49.24 & 0.201310 & 0.065243 & -99.9 & 15.85 & 13.31 & -99.9 & -99.9 & -99.9 & -99.9 & 13.32 & 0.48 & -99.9 & IRR & 1 \\
NV098 & 17:45:50.65 & -28:48:17.95 & 0.137573 & 0.026396 & -99.9 & 16.85 & 13.71 & -99.9 & 10.61 & -99.9 & -99.9 & 13.84 & 0.67 & -99.9 & IRR & -99.9 \\
NV099 & 17:45:50.85 & -28:50:20.91 & 0.108777 & 0.008018 & -99.9 & -99.9 & 13.36 & -99.9 & 9.4 & 8.73 & 8.96 & 12.99 & 0.69 & -99.9 & IRR & -99.9 \\
NV100 & 17:45:50.87 & -28:48:11.55 & 0.139511 & 0.026633 & -99.9 & 14.69 & 11.63 & 10.42 & -99.9 & -99.9 & -99.9 & 11.87 & 0.37 & -99.9 & IRR & -99.9 \\
NV101 & 17:45:51.02 & -28:49:07.85 & 0.126429 & 0.018051 & -99.9 & 15.52 & 11.77 & 10.27 & 9.23 & 8.89 & -99.9 & 11.67 & 0.57 & -99.9 & IRR & -99.9 \\
NV102 & 17:45:51.05 & -28:45:41.88 & 0.175338 & 0.047736 & -99.9 & 15.46 & 13.07 & -99.9 & 11.2 & 10.93 & -99.9 & 13.21 & 0.53 & 985 & SR & -99.9 \\
NV103 & 17:45:51.05 & -28:48:07.19 & 0.140889 & 0.026703 & -99.9 & -99.9 & 15.88 & -99.9 & -99.9 & -99.9 & -99.9 & 15.85 & 1.43 & 647 & Mira & -99.9 \\
NV104 & 17:45:51.08 & -28:47:01.30 & 0.156569 & 0.036141 & -99.9 & -99.9 & 15.14 & -99.9 & -99.9 & -99.9 & -99.9 & 14.87 & 1.46 & 1047 & SR & -99.9 \\
NV105 & 17:45:51.11 & -28:53:55.26 & 0.058437 & -0.02379 & -99.9 & 15.65 & 12.28 & 10.62 & 9.89 & 9.78 & -99.9 & 12.28 & 0.86 & -99.9 & IRR & -99.9 \\
NV106 & 17:45:51.23 & -28:54:57.50 & 0.043905 & -0.03317 & -99.9 & 16.50 & 12.65 & 7.34 & 6.1 & 5.12 & 4.77 & 12.81 & 2.17 & 438 & Mira & 1 \\
NV107 & 17:45:51.24 & -28:45:04.30 & 0.184623 & 0.052559 & -99.9 & 16.69 & 14.27 & -99.9 & -99.9 & -99.9 & -99.9 & 14.29 & 1.16 & -99.9 & Microlensing? & -99.9 \\
NV108 & 17:45:51.30 & -28:47:05.36 & 0.156015 & 0.034883 & -99.9 & 17.35 & 14.53 & -99.9 & -99.9 & -99.9 & -99.9 & 14.85 & 2.19 & -99.9 & RCB? & -99.9 \\
NV109 & 17:45:51.32 & -28:42:22.32 & 0.223190 & 0.075739 & 18.35 & 15.23 & 13.49 & -99.9 & -99.9 & -99.9 & -99.9 & 13.51 & 0.48 & -99.9 & LPV & -99.9 \\
NV110 & 17:45:51.45 & -28:55:06.60 & 0.042161 & -0.03516 & -99.9 & 15.53 & -99.9 & 9.1 & 7.81 & 7.26 & 7.36 & 11.52 & 0.79 & 464 & SR & 1 \\
NV111 & 17:45:51.45 & -28:50:22.35 & 0.109593 & 0.005909 & -99.9 & 18.42 & 14.93 & -99.9 & -99.9 & -99.9 & -99.9 & 15.54 & 1.2 & 1391 & LTV & -99.9 \\
NV112 & 17:45:51.56 & -28:48:23.99 & 0.137856 & 0.022711 & -99.9 & 18.16 & 13.54 & 12.07 & 10.86 & 10.8 & -99.9 & 13.6 & 1.12 & -99.9 & LPV & -99.9 \\
NV113 & 17:45:51.64 & -28:48:03.40 & 0.142906 & 0.025413 & -99.9 & 18.10 & 13.36 & 11.46 & 10.48 & -99.9 & -99.9 & 13.13 & 0.61 & -99.9 & IRR & -99.9 \\
NV114 & 17:45:51.78 & -28:42:23.77 & 0.223722 & 0.074090 & -99.9 & 16.89 & 14.18 & -99.9 & -99.9 & -99.9 & -99.9 & 14.29 & 0.86 & 1438 & SR & -99.9 \\
NV115 & 17:45:51.81 & -28:45:51.01 & 0.174628 & 0.044032 & 18.64 & 14.47 & 12.25 & 10.87 & 10.67 & 10.15 & -99.9 & 12.51 & 1.2 & -99.9 & RCB? & -99.9 \\
NV116 & 17:45:51.85 & -28:47:44.86 & 0.147700 & 0.027445 & -99.9 & 16.01 & 12.43 & 10.81 & -99.9 & -99.9 & -99.9 & 12.62 & 0.54 & 1648 & SR & -99.9 \\
NV117 & 17:45:51.84 & -28:47:50.10 & 0.146443 & 0.026712 & 18.99 & 15.57 & 12.10 & 9.95 & 9.14 & 8.16 & -99.9 & 11.76 & 0.5 & -99.9 & IRR & -99.9 \\
NV118 & 17:45:51.92 & -28:44:51.70 & 0.188889 & 0.052290 & -99.9 & -99.9 & 15.35 & 8.0 & 6.37 & 5.06 & 4.48 & 14.1 & 3.18 & 937 & Mira & 1 \\
NV119 & 17:45:52.09 & -28:48:40.05 & 0.135060 & 0.018727 & -99.9 & 17.11 & 13.14 & 11.31 & 10.4 & 10.04 & -99.9 & 12.71 & 0.56 & 1179 & SR & -99.9 \\
NV120 & 17:45:52.10 & -28:50:47.54 & 0.104847 & 0.000252 & -99.9 & 16.60 & 13.11 & -99.9 & -99.9 & -99.9 & -99.9 & 13.28 & 0.76 & -99.9 & IRR & -99.9 \\
NV121 & 17:45:52.24 & -28:42:21.13 & 0.225209 & 0.073059 & -99.9 & 15.90 & 13.32 & 12.55 & 11.87 & -99.9 & -99.9 & 13.53 & 0.73 & 761 & SR & -99.9 \\
NV122 & 17:45:52.26 & -28:42:26.44 & 0.223989 & 0.072228 & -99.9 & 17.69 & 14.96 & -99.9 & -99.9 & -99.9 & -99.9 & 15.45 & 1.83 & -99.9 & Fader & -99.9 \\
NV123 & 17:45:52.32 & -28:42:59.41 & 0.216298 & 0.067250 & 19.13 & 15.48 & 13.47 & -99.9 & -99.9 & -99.9 & -99.9 & 13.58 & 0.54 & -99.9 & LPV & -99.9 \\
NV124 & 17:45:52.33 & -28:48:42.63 & 0.134900 & 0.017616 & 17.14 & 14.55 & 12.76 & 12.75 & 12.15 & -99.9 & -99.9 & 12.53 & 1.04 & -99.9 & LPV/Microlensing & 1 \\
NV125 & 17:45:52.43 & -28:43:45.63 & 0.205543 & 0.060230 & -99.9 & -99.9 & 15.02 & -99.9 & -99.9 & -99.9 & -99.9 & 15.0 & 1.62 & -99.9 & Eruptive/FUor? & -99.9 \\
NV126 & 17:45:52.51 & -28:42:27.05 & 0.224330 & 0.071343 & -99.9 & -99.9 & 16.16 & -99.9 & -99.9 & -99.9 & -99.9 & 15.41 & 1.34 & -99.9 & Dipper & -99.9 \\
NV127 & 17:45:52.56 & -28:43:49.75 & 0.204811 & 0.059228 & -99.9 & -99.9 & 14.73 & -99.9 & -99.9 & -99.9 & -99.9 & 15.2 & 1.93 & -99.9 & Dipper & -99.9 \\
NV128 & 17:45:52.71 & -28:48:17.97 & 0.141475 & 0.019988 & -99.9 & 15.85 & 11.76 & -99.9 & 9.13 & 8.66 & -99.9 & 11.91 & 0.73 & -99.9 & IRR & -99.9 \\
NV129 & 17:45:52.80 & -28:44:08.15 & 0.200895 & 0.055834 & -99.9 & -99.9 & 13.15 & 10.65 & 10.3 & 9.95 & -99.9 & 13.39 & 0.69 & -99.9 & IRR & -99.9 \\
NV130 & 17:45:53.01 & -28:49:30.23 & 0.124903 & 0.008612 & -99.9 & 15.39 & 12.59 & 11.95 & 11.37 & 10.0 & -99.9 & 12.77 & 0.54 & -99.9 & IRR & -99.9 \\
NV131 & 17:45:53.06 & -28:42:51.30 & 0.219621 & 0.066130 & -99.9 & 15.93 & 12.78 & 11.58 & 10.7 & 10.06 & -99.9 & 12.23 & 0.86 & -99.9 & LPV & -99.9 \\
NV132 & 17:45:53.26 & -28:51:57.95 & 0.090347 & -0.01353 & -99.9 & 17.22 & 13.07 & 11.07 & 10.1 & -99.9 & -99.9 & 13.21 & 0.56 & 755 & SR & -99.9 \\
NV133 & 17:45:53.30 & -28:49:06.20 & 0.131158 & 0.011174 & -99.9 & 15.78 & 13.15 & -99.9 & -99.9 & -99.9 & -99.9 & 13.06 & 0.72 & -99.9 & LPV & -99.9 \\
NV134 & 17:45:53.48 & -28:48:48.28 & 0.135757 & 0.013191 & -99.9 & 16.12 & 13.47 & 12.69 & 12.14 & 10.37 & -99.9 & 13.36 & 1.12 & -99.9 & LPV & -99.9 \\
NV135 & 17:45:53.52 & -28:47:41.18 & 0.151751 & 0.022768 & 18.67 & 14.93 & 11.70 & 10.78 & 9.75 & 9.91 & -99.9 & 11.95 & 0.71 & -99.9 & IRR & -99.9 \\
NV136 & 17:45:53.90 & -28:44:23.04 & 0.199462 & 0.050237 & -99.9 & 15.50 & 12.28 & 10.86 & 10.28 & -99.9 & -99.9 & 12.15 & 0.47 & -99.9 & IRR & -99.9 \\
NV137 & 17:45:53.91 & -28:46:59.64 & 0.162329 & 0.027582 & -99.9 & 14.90 & 11.93 & -99.9 & -99.9 & 9.26 & -99.9 & 11.79 & 0.26 & -99.9 & IRR & 1 \\
NV138 & 17:45:53.90 & -28:53:52.82 & 0.064328 & -0.03215 & -99.9 & 16.87 & 13.46 & 11.33 & 10.69 & 9.9 & -99.9 & 13.37 & 0.44 & 1641 & SR & -99.9 \\
NV139 & 17:45:53.96 & -28:45:56.72 & 0.177355 & 0.036508 & -99.9 & 16.36 & 13.94 & -99.9 & -99.9 & -99.9 & -99.9 & 14.34 & 1.6 & -99.9 & Dipper & -99.9 \\
NV140 & 17:45:54.06 & -28:45:42.94 & 0.180804 & 0.038205 & -99.9 & 15.64 & 13.18 & 12.0 & 11.5 & 10.74 & -99.9 & 13.33 & 0.44 & -99.9 & IRR & -99.9 \\
NV141 & 17:45:54.06 & -28:53:54.10 & 0.064317 & -0.03281 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & 14.62 & 2.26 & -99.9 & Eruptive/EXor & -99.9 \\
NV142 & 17:45:54.12 & -28:45:03.32 & 0.190331 & 0.043721 & 17.35 & 14.28 & 12.49 & 11.65 & 11.32 & -99.9 & -99.9 & 12.75 & 0.61 & 15.566 & CepII & 2 \\
NV143 & 17:45:54.12 & -28:50:51.63 & 0.107712 & -0.00662 & -99.9 & 14.93 & 12.44 & -99.9 & -99.9 & -99.9 & -99.9 & 12.52 & 0.34 & -99.9 & IRR & 1 \\
NV144 & 17:45:54.40 & -28:43:52.29 & 0.207704 & 0.053128 & -99.9 & -99.9 & 16.45 & -99.9 & -99.9 & -99.9 & -99.9 & 15.82 & 1.04 & -99.9 & Eruptive/Fader? & -99.9 \\
NV145 & 17:45:54.41 & -28:54:44.22 & 0.053100 & -0.04116 & -99.9 & 16.01 & 12.25 & 10.71 & 9.67 & 9.02 & -99.9 & 12.17 & 0.71 & -99.9 & IRR & -99.9 \\
NV146 & 17:45:54.44 & -28:43:57.79 & 0.206472 & 0.052212 & 16.86 & 16.15 & 15.18 & -99.9 & -99.9 & -99.9 & -99.9 & 15.31 & 1.29 & 797 & LTV & -99.9 \\
NV147 & 17:45:54.47 & -28:43:21.43 & 0.215154 & 0.057378 & -99.9 & 17.25 & 15.03 & -99.9 & -99.9 & -99.9 & -99.9 & 15.34 & 1.22 & -99.9 & Dipper & -99.9 \\
NV148 & 17:45:54.56 & -28:43:35.55 & 0.211976 & 0.055056 & -99.9 & -99.9 & 15.53 & -99.9 & -99.9 & -99.9 & -99.9 & 15.43 & 1.09 & -99.9 & Dipper & -99.9 \\
NV149 & 17:45:54.69 & -28:51:52.92 & 0.094258 & -0.01726 & 19.28 & 14.40 & 11.55 & 9.62 & 9.51 & 8.41 & 7.95 & 11.76 & 0.46 & -99.9 & IRR & 1 \\
NV150 & 17:45:54.83 & -28:54:38.25 & 0.055301 & -0.04159 & 18.37 & 15.14 & 13.32 & 11.81 & 11.23 & -99.9 & -99.9 & 13.31 & 0.32 & 10.267 & CepII & 2 \\
NV151 & 17:45:54.84 & -28:54:41.25 & 0.054613 & -0.04206 & -99.9 & 17.81 & 14.67 & -99.9 & -99.9 & -99.9 & -99.9 & 14.45 & 0.65 & -99.9 & IRR & -99.9 \\
NV152 & 17:45:54.86 & -28:48:38.47 & 0.140707 & 0.010308 & -99.9 & -99.9 & 15.37 & -99.9 & -99.9 & -99.9 & -99.9 & 15.69 & 1.16 & 964 & LTV & -99.9 \\
NV153 & 17:45:54.91 & -28:46:54.12 & 0.165555 & 0.025233 & -99.9 & 16.16 & 13.36 & -99.9 & -99.9 & 10.08 & -99.9 & 13.71 & 0.76 & -99.9 & IRR & -99.9 \\
NV154 & 17:45:55.06 & -28:44:06.12 & 0.205685 & 0.049059 & -99.9 & 17.13 & 14.32 & -99.9 & -99.9 & -99.9 & -99.9 & 14.2 & 0.92 & 525 & SR & -99.9 \\
NV155 & 17:45:55.16 & -28:44:19.16 & 0.202778 & 0.046870 & -99.9 & 16.13 & 13.00 & 12.13 & 11.18 & -99.9 & -99.9 & 13.37 & 0.72 & -99.9 & IRR & -99.9 \\
NV156 & 17:45:55.20 & -28:52:04.54 & 0.092466 & -0.02052 & -99.9 & 16.85 & 13.98 & -99.9 & -99.9 & -99.9 & -99.9 & 13.97 & 0.76 & -99.9 & IRR & -99.9 \\
NV157 & 17:45:55.22 & -28:48:44.01 & 0.140074 & 0.008388 & -99.9 & 15.09 & 11.74 & -99.9 & -99.9 & -99.9 & -99.9 & 11.72 & 0.79 & -99.9 & IRR & 1 \\
NV158 & 17:45:55.27 & -28:47:12.01 & 0.161986 & 0.021541 & -99.9 & 16.51 & 14.00 & 12.94 & 12.03 & -99.9 & -99.9 & 14.0 & 0.69 & -99.9 & IRR & -99.9 \\
NV159 & 17:45:55.30 & -28:47:56.14 & 0.151577 & 0.015067 & -99.9 & -99.9 & 14.52 & -99.9 & -99.9 & -99.9 & -99.9 & 14.83 & 1.16 & -99.9 & IRR & -99.9 \\
NV160 & 17:45:55.49 & -28:46:16.96 & 0.175456 & 0.028824 & -99.9 & 16.41 & 12.42 & 10.86 & 10.14 & 9.88 & -99.9 & 12.19 & 0.41 & 701 & SR & 1 \\
NV161 & 17:45:55.62 & -28:44:14.08 & 0.204854 & 0.046175 & -99.9 & -99.9 & 15.24 & -99.9 & -99.9 & -99.9 & -99.9 & 14.94 & 1.25 & -99.9 & LPV & -99.9 \\
NV162 & 17:45:55.61 & -28:46:32.24 & 0.172073 & 0.026219 & 18.84 & 14.15 & 11.58 & 10.47 & 10.13 & 9.5 & -99.9 & 11.46 & 0.22 & -99.9 & IRR & 1 \\
NV163 & 17:45:55.60 & -28:48:21.01 & 0.146258 & 0.010520 & -99.9 & 15.60 & 12.31 & -99.9 & -99.9 & 9.36 & -99.9 & 12.45 & 0.51 & -99.9 & IRR & -99.9 \\
NV164 & 17:45:55.65 & -28:49:50.26 & 0.125165 & -0.00250 & -99.9 & 16.17 & 12.84 & 11.3 & 10.53 & 10.07 & -99.9 & 13.52 & 1.19 & -99.9 & IRR & -99.9 \\
NV165 & 17:45:55.74 & -28:49:33.17 & 0.129394 & -0.00032 & -99.9 & -99.9 & 13.95 & 11.98 & 11.21 & 10.5 & -99.9 & 14.05 & 1.18 & 1276 & SR & -99.9 \\
NV166 & 17:45:55.82 & -28:45:18.68 & 0.189909 & 0.036218 & -99.9 & 16.61 & 12.39 & 7.16 & 5.8 & 4.56 & 3.98 & 12.89 & 2.3 & 546 & Mira & 1 \\
NV167 & 17:45:55.80 & -28:53:11.11 & 0.077811 & -0.03201 & -99.9 & 15.20 & 11.89 & 10.86 & 9.94 & 9.9 & -99.9 & 11.94 & 0.32 & -99.9 & IRR & -99.9 \\
NV168 & 17:45:55.85 & -28:47:21.24 & 0.160896 & 0.018406 & -99.9 & 15.48 & 12.71 & -99.9 & -99.9 & -99.9 & -99.9 & 13.03 & 0.42 & 211 & SR & -99.9 \\
NV169 & 17:45:55.91 & -28:47:04.69 & 0.164940 & 0.020603 & -99.9 & 16.55 & 13.96 & -99.9 & -99.9 & -99.9 & -99.9 & 14.16 & 0.85 & 1571 & SR & -99.9 \\
NV170 & 17:45:55.91 & -28:47:26.87 & 0.159688 & 0.017382 & -99.9 & -99.9 & 15.13 & 12.04 & 11.4 & -99.9 & -99.9 & 15.43 & 1.37 & -99.9 & Eruptive & -99.9 \\
NV171 & 17:45:56.03 & -28:49:42.75 & 0.127675 & -0.00261 & -99.9 & 18.25 & 15.24 & -99.9 & -99.9 & -99.9 & -99.9 & 15.34 & 1.25 & -99.9 & Dipper & -99.9 \\
NV172 & 17:45:56.14 & -28:54:02.81 & 0.066205 & -0.04056 & -99.9 & 16.91 & 12.63 & 11.83 & 9.76 & 9.22 & -99.9 & 12.65 & 0.28 & -99.9 & IRR & -99.9 \\
NV173 & 17:45:56.24 & -28:50:22.01 & 0.118760 & -0.00894 & -99.9 & 14.91 & 12.34 & 11.13 & 10.82 & 10.39 & -99.9 & 12.6 & 0.64 & -99.9 & IRR & -99.9 \\
NV174 & 17:45:56.35 & -28:46:27.98 & 0.174491 & 0.024523 & -99.9 & 14.53 & 11.63 & 10.55 & 9.83 & 9.47 & -99.9 & 11.68 & 0.34 & -99.9 & IRR & 1 \\
NV175 & 17:45:56.36 & -28:51:31.99 & 0.102387 & -0.01942 & -99.9 & 17.19 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & 13.61 & 0.5 & -99.9 & LPV & -99.9 \\
NV176 & 17:45:56.36 & -28:53:27.89 & 0.074909 & -0.03620 & -99.9 & -99.9 & -99.9 & -99.9 & 7.67 & 7.05 & 7.26 & 12.18 & 1.2 & 511 & SR & 1 \\
NV177 & 17:45:56.37 & -28:54:13.35 & 0.064132 & -0.04279 & -99.9 & 16.11 & 12.81 & -99.9 & -99.9 & -99.9 & -99.9 & 12.82 & 0.58 & -99.9 & IRR & -99.9 \\
NV178 & 17:45:56.51 & -28:45:02.58 & 0.195049 & 0.036378 & 19.28 & 15.19 & -99.9 & 11.35 & 10.78 & -99.9 & -99.9 & 12.53 & 0.36 & 1333 & SR & -99.9 \\
NV179 & 17:45:56.53 & -28:46:28.91 & 0.174603 & 0.023844 & -99.9 & 15.05 & 12.31 & -99.9 & -99.9 & 9.71 & -99.9 & 12.19 & 0.4 & -99.9 & IRR & -99.9 \\
NV180 & 17:45:56.59 & -28:47:55.49 & 0.154181 & 0.011142 & -99.9 & 16.23 & 12.38 & -99.9 & -99.9 & -99.9 & 9.22 & 12.27 & 0.48 & 1071 & SR & 1 \\
NV181 & 17:45:56.62 & -28:48:33.08 & 0.145328 & 0.005606 & -99.9 & 15.62 & 12.15 & -99.9 & 10.08 & 9.96 & -99.9 & 12.15 & 0.26 & 1331 & SR & 1 \\
NV182 & 17:45:56.69 & -28:45:59.31 & 0.181939 & 0.027609 & -99.9 & 17.53 & 13.69 & -99.9 & -99.9 & -99.9 & -99.9 & 13.64 & 0.79 & -99.9 & LPV & -99.9 \\
NV183 & 17:45:56.82 & -28:44:33.72 & 0.202471 & 0.039601 & -99.9 & 17.07 & 14.64 & -99.9 & -99.9 & -99.9 & -99.9 & 14.8 & 0.89 & -99.9 & LPV & -99.9 \\
NV184 & 17:45:56.85 & -28:53:38.83 & 0.073233 & -0.03930 & -99.9 & 15.18 & 12.22 & 11.58 & 10.63 & 10.51 & -99.9 & 12.37 & 0.33 & 491 & SR & -99.9 \\
NV185 & 17:45:56.91 & -28:47:35.93 & 0.159439 & 0.012956 & -99.9 & -99.9 & 16.45 & -99.9 & -99.9 & -99.9 & -99.9 & 15.43 & 1.55 & -99.9 & Eruptive/FUor & -99.9 \\
NV186 & 17:45:56.98 & -28:52:24.22 & 0.091179 & -0.02891 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & 16.09 & 1.2 & -99.9 & Eruptive & -99.9 \\
NV187 & 17:45:57.08 & -28:46:54.48 & 0.169581 & 0.018434 & -99.9 & 17.79 & 13.00 & 11.32 & 10.1 & 9.77 & -99.9 & 13.18 & 0.72 & -99.9 & IRR & -99.9 \\
NV188 & 17:45:57.16 & -28:53:44.29 & 0.072539 & -0.04107 & -99.9 & 15.46 & -99.9 & -99.9 & 8.57 & 8.11 & 8.1 & 12.15 & 0.75 & 407 & Mira & 1 \\
NV189 & 17:45:57.63 & -28:55:19.56 & 0.050828 & -0.05630 & -99.9 & 16.75 & 14.05 & -99.9 & -99.9 & -99.9 & -99.9 & 13.99 & 0.73 & -99.9 & IRR & -99.9 \\
NV190 & 17:45:57.93 & -28:50:51.99 & 0.114867 & -0.01856 & -99.9 & -99.9 & 15.03 & -99.9 & -99.9 & -99.9 & -99.9 & 14.57 & 0.79 & -99.9 & IRR & -99.9 \\
NV191 & 17:45:57.96 & -28:45:39.20 & 0.189121 & 0.026557 & -99.9 & 14.75 & 11.51 & 10.16 & 9.56 & 9.2 & -99.9 & 11.55 & 0.32 & -99.9 & IRR & -99.9 \\
NV192 & 17:45:57.97 & -28:48:39.64 & 0.146328 & 0.000463 & -99.9 & 15.83 & 12.21 & 10.57 & 9.47 & 9.0 & -99.9 & 12.22 & 0.43 & -99.9 & IRR & -99.9 \\
NV193 & 17:45:58.15 & -28:51:58.45 & 0.099520 & -0.02885 & -99.9 & 16.60 & 13.28 & 12.15 & 11.15 & -99.9 & -99.9 & 13.63 & 1.02 & -99.9 & LPV & -99.9 \\
NV194 & 17:45:58.23 & -28:53:34.67 & 0.076853 & -0.04301 & -99.9 & 14.50 & -99.9 & -99.9 & 9.51 & 9.22 & 9.51 & 11.5 & 0.53 & -99.9 & IRR & -99.9 \\
NV195 & 17:45:58.39 & -28:44:26.86 & 0.207097 & 0.035675 & 18.06 & 17.09 & 14.80 & -99.9 & -99.9 & -99.9 & -99.9 & 14.45 & 1.1 & -99.9 & LPV & -99.9 \\
NV196 & 17:45:58.50 & -28:44:26.68 & 0.207339 & 0.035371 & -99.9 & -99.9 & 14.16 & -99.9 & -99.9 & -99.9 & -99.9 & 13.56 & 0.98 & -99.9 & LPV & -99.9 \\
NV197 & 17:45:58.64 & -28:46:06.05 & 0.184031 & 0.020577 & 18.10 & 13.87 & -99.9 & 10.39 & 10.02 & 9.8 & -99.9 & 11.58 & 0.25 & -99.9 & IRR & -99.9 \\
NV198 & 17:45:58.98 & -28:49:49.20 & 0.131758 & -0.01275 & -99.9 & 16.21 & 13.15 & 12.52 & 11.78 & -99.9 & -99.9 & 13.01 & 0.78 & 1549 & SR & -99.9 \\
NV199 & 17:45:59.20 & -28:53:57.88 & 0.073179 & -0.04937 & -99.9 & 14.60 & 12.02 & 11.39 & 10.89 & 9.81 & -99.9 & 12.04 & 0.32 & 1236 & SR & -99.9 \\
NV200 & 17:45:59.53 & -28:46:00.92 & 0.186955 & 0.018517 & -99.9 & 18.41 & 15.29 & -99.9 & -99.9 & -99.9 & -99.9 & 15.43 & 1.26 & -99.9 & Eruptive & -99.9 \\
NV201 & 17:45:59.58 & -28:46:33.94 & 0.179219 & 0.013588 & -99.9 & 15.82 & 12.44 & 11.29 & 10.35 & 9.55 & -99.9 & 12.44 & 0.37 & -99.9 & IRR & 1 \\
NV202 & 17:45:59.60 & -28:46:45.89 & 0.176409 & 0.011820 & -99.9 & 17.65 & 13.92 & 11.63 & 11.1 & 9.82 & -99.9 & 13.96 & 0.75 & 474 & SR & -99.9 \\
NV203 & 17:45:59.67 & -28:43:52.07 & 0.217775 & 0.036720 & -99.9 & -99.9 & 15.10 & -99.9 & -99.9 & -99.9 & -99.9 & 14.89 & 1.43 & -99.9 & LPV & -99.9 \\
NV204 & 17:45:59.72 & -28:55:45.93 & 0.048549 & -0.06663 & -99.9 & 15.21 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & 11.64 & 0.63 & -99.9 & IRR & -99.9 \\
NV205 & 17:45:59.95 & -28:51:32.00 & 0.109203 & -0.03062 & -99.9 & 15.90 & 13.26 & 12.25 & 12.22 & -99.9 & -99.9 & 13.35 & 0.44 & -99.9 & LPV & -99.9 \\
NV206 & 17:46:00.39 & -28:48:31.34 & 0.152906 & -0.00590 & 19.18 & 15.74 & 13.47 & -99.9 & 11.51 & -99.9 & -99.9 & 13.58 & 0.88 & -99.9 & IRR & -99.9 \\
NV207 & 17:46:00.44 & -28:47:47.63 & 0.163359 & 0.000276 & -99.9 & 14.53 & 11.85 & 10.56 & -99.9 & 9.36 & -99.9 & 11.95 & 0.32 & 1218 & SR & 1 \\
NV208 & 17:46:00.58 & -28:48:11.67 & 0.157926 & -0.00364 & -99.9 & 14.65 & 11.75 & 10.95 & 10.2 & 9.77 & -99.9 & 12.02 & 0.4 & -99.9 & IRR & -99.9 \\
NV209 & 17:46:00.59 & -28:54:51.36 & 0.063127 & -0.06143 & -99.9 & -99.9 & 13.56 & 11.57 & 11.03 & -99.9 & -99.9 & 13.01 & 0.81 & -99.9 & IRR & -99.9 \\
NV210 & 17:46:00.67 & -28:50:19.98 & 0.127662 & -0.02247 & -99.9 & 15.55 & 12.51 & -99.9 & -99.9 & -99.9 & -99.9 & 12.53 & 0.52 & -99.9 & IRR & -99.9 \\
NV211 & 17:46:00.87 & -28:47:19.32 & 0.170888 & 0.003033 & -99.9 & 17.65 & 13.54 & 12.68 & 10.79 & 10.29 & -99.9 & 13.6 & 0.73 & 968 & SR & -99.9 \\
NV212 & 17:46:01.00 & -28:51:06.82 & 0.117178 & -0.03026 & 16.70 & 14.70 & 12.33 & -99.9 & -99.9 & -99.9 & -99.9 & 12.52 & 0.5 & -99.9 & IRR & -99.9 \\
NV213 & 17:46:01.21 & -28:56:17.08 & 0.043977 & -0.07576 & -99.9 & 14.96 & 12.29 & 11.3 & -99.9 & -99.9 & -99.9 & 12.47 & 0.89 & 698 & SR & -99.9 \\
NV214 & 17:46:01.28 & -28:53:38.04 & 0.081845 & -0.05300 & -99.9 & 15.85 & 13.24 & 12.53 & 11.81 & -99.9 & -99.9 & 13.38 & 1.22 & -99.9 & IRR & -99.9 \\
NV215 & 17:46:01.30 & -28:46:04.09 & 0.189561 & 0.012548 & -99.9 & 17.57 & 13.04 & 11.13 & 10.09 & 10.21 & -99.9 & 12.4 & 0.79 & -99.9 & IRR & -99.9 \\
NV216 & 17:46:01.33 & -28:43:37.96 & 0.224290 & 0.033563 & 18.33 & 13.75 & 11.35 & 9.77 & 9.36 & 8.91 & -99.9 & 11.33 & 0.53 & 121 & SR & 1 \\
NV217 & 17:46:01.36 & -28:50:19.28 & 0.129136 & -0.02451 & -99.9 & 16.56 & 14.23 & -99.9 & -99.9 & -99.9 & -99.9 & 14.13 & 0.81 & 534 & LTV & -99.9 \\
NV218 & 17:46:01.39 & -28:48:08.87 & 0.160132 & -0.00576 & 18.83 & 15.92 & 13.67 & 12.04 & 11.65 & -99.9 & -99.9 & 13.56 & 0.56 & -99.9 & IRR & -99.9 \\
NV219 & 17:46:01.50 & -28:46:43.53 & 0.180576 & 0.006239 & -99.9 & -99.9 & 15.24 & -99.9 & -99.9 & -99.9 & -99.9 & 15.38 & 1.19 & -99.9 & Dipper & -99.9 \\
NV220 & 17:46:01.63 & -28:44:08.96 & 0.217489 & 0.028174 & -99.9 & 16.75 & 13.90 & -99.9 & -99.9 & -99.9 & -99.9 & 14.1 & 0.97 & -99.9 & LPV & -99.9 \\
NV221 & 17:46:01.63 & -28:48:40.13 & 0.153167 & -0.01102 & -99.9 & 15.00 & 11.69 & 9.8 & 9.19 & 8.77 & -99.9 & 11.78 & 0.39 & -99.9 & IRR & -99.9 \\
NV222 & 17:46:01.68 & -28:46:01.51 & 0.190898 & 0.011730 & 18.89 & 14.35 & 11.86 & 9.85 & 9.3 & 8.93 & 8.93 & 11.69 & 0.73 & 97.16 & Mira & 1 \\
NV223 & 17:46:02.12 & -28:50:06.96 & 0.133510 & -0.02511 & -99.9 & -99.9 & 15.22 & 12.46 & 11.46 & -99.9 & -99.9 & 14.39 & 1.14 & -99.9 & IRR & -99.9 \\
NV224 & 17:46:02.15 & -28:47:35.08 & 0.169595 & -0.00325 & -99.9 & 14.95 & 12.17 & -99.9 & 10.51 & -99.9 & -99.9 & 12.23 & 0.38 & -99.9 & IRR & -99.9 \\
NV225 & 17:46:02.40 & -28:50:19.99 & 0.130939 & -0.02785 & -99.9 & 15.46 & 12.28 & -99.9 & 10.6 & -99.9 & -99.9 & 12.34 & 0.28 & -99.9 & IRR & -99.9 \\
NV226 & 17:46:02.43 & -28:43:19.32 & 0.230799 & 0.032831 & -99.9 & 15.60 & -99.9 & 8.13 & 6.41 & 5.24 & 4.9 & 11.92 & 1.16 & 428 & Mira & -99.9 \\
NV227 & 17:46:02.47 & -28:46:01.19 & 0.192476 & 0.009310 & -99.9 & 16.74 & 12.53 & 10.95 & 9.86 & 9.21 & -99.9 & 12.63 & 0.52 & 440 & SR & -99.9 \\
NV228 & 17:46:02.47 & -28:54:36.07 & 0.070325 & -0.06508 & -99.9 & 17.34 & 13.66 & -99.9 & 10.4 & 9.6 & -99.9 & 14.23 & 1.36 & -99.9 & IRR & -99.9 \\
NV229 & 17:46:02.62 & -28:45:53.67 & 0.194530 & 0.009954 & -99.9 & -99.9 & 12.39 & 10.03 & 8.91 & 8.31 & 7.76 & 12.47 & 0.73 & 1378 & SR & -99.9 \\
NV230 & 17:46:02.66 & -28:51:07.79 & 0.120107 & -0.03559 & -99.9 & 15.76 & 12.50 & -99.9 & 10.26 & 10.06 & -99.9 & 12.55 & 0.47 & 1069 & SR & -99.9 \\
NV231 & 17:46:02.88 & -28:44:20.92 & 0.217032 & 0.022537 & -99.9 & 16.70 & 13.96 & 8.54 & 6.76 & 5.49 & 4.77 & 14.13 & 1.64 & 465 & Mira & -99.9 \\
NV232 & 17:46:02.97 & -28:48:45.47 & 0.154446 & -0.01597 & -99.9 & 16.72 & 12.78 & -99.9 & 9.62 & 9.31 & -99.9 & 12.69 & 2.88 & 1291 & RCB/DYPer? & -99.9 \\
NV233 & 17:46:03.04 & -28:45:50.16 & 0.196173 & 0.009132 & -99.9 & -99.9 & 14.58 & 12.73 & 12.05 & -99.9 & -99.9 & 15.9 & 2.46 & -99.9 & Dipper & -99.9 \\
NV234 & 17:46:03.65 & -28:43:49.70 & 0.225913 & 0.024632 & 16.74 & 14.91 & 13.44 & 12.58 & 11.69 & -99.9 & -99.9 & 13.39 & 0.69 & -99.9 & Microlensing & -99.9 \\
NV235 & 17:46:03.66 & -28:48:11.97 & 0.163714 & -0.01330 & 19.26 & 16.34 & 12.53 & -99.9 & -99.9 & -99.9 & -99.9 & 13.1 & 2.29 & -99.9 & RCB? & 1 \\
NV236 & 17:46:03.67 & -28:47:58.83 & 0.166838 & -0.01141 & -99.9 & 15.39 & 11.78 & -99.9 & -99.9 & -99.9 & -99.9 & 11.89 & 0.92 & -99.9 & IRR & -99.9 \\
NV237 & 17:46:03.93 & -28:45:38.53 & 0.200626 & 0.008031 & -99.9 & 17.66 & 15.38 & -99.9 & -99.9 & -99.9 & -99.9 & 15.63 & 1.1 & -99.9 & Fader & -99.9 \\
NV238 & 17:46:03.97 & -28:46:46.70 & 0.184521 & -0.00192 & -99.9 & 17.09 & 12.84 & 11.28 & 10.24 & 9.79 & -99.9 & 12.76 & 0.55 & 477 & SR & -99.9 \\
NV239 & 17:46:03.99 & -28:51:53.69 & 0.111738 & -0.04636 & 18.62 & 14.78 & 12.26 & -99.9 & 10.91 & 10.45 & -99.9 & 12.51 & 0.69 & 922 & SR & -99.9 \\
NV240 & 17:46:04.02 & -28:50:00.63 & 0.138606 & -0.03010 & -99.9 & 18.12 & 15.25 & -99.9 & -99.9 & -99.9 & -99.9 & 16.0 & 1.43 & -99.9 & Fader & -99.9 \\
NV241 & 17:46:04.05 & -28:52:57.10 & 0.096803 & -0.05570 & -99.9 & 16.87 & 14.44 & -99.9 & -99.9 & -99.9 & -99.9 & 15.07 & 1.5 & -99.9 & Fader & -99.9 \\
NV242 & 17:46:04.06 & -28:50:12.84 & 0.135786 & -0.03199 & -99.9 & -99.9 & 14.56 & -99.9 & -99.9 & -99.9 & -99.9 & 13.76 & 1.73 & -99.9 & LPV & -99.9 \\
NV243 & 17:46:04.14 & -28:49:17.21 & 0.149138 & -0.02420 & -99.9 & 15.86 & 13.05 & 11.21 & 10.95 & -99.9 & -99.9 & 13.13 & 0.53 & -99.9 & IRR & -99.9 \\
NV244 & 17:46:04.54 & -28:47:47.18 & 0.171252 & -0.01243 & -99.9 & 15.68 & 12.92 & -99.9 & -99.9 & -99.9 & -99.9 & 12.95 & 0.46 & -99.9 & IRR & -99.9 \\
NV245 & 17:46:04.74 & -28:44:55.41 & 0.212385 & 0.011752 & -99.9 & 18.38 & 14.61 & -99.9 & -99.9 & -99.9 & -99.9 & 14.3 & 0.89 & -99.9 & LPV & -99.9 \\
NV246 & 17:46:04.83 & -28:46:30.94 & 0.189892 & -0.00232 & -99.9 & -99.9 & 15.60 & -99.9 & -99.9 & -99.9 & -99.9 & 15.67 & 1.17 & -99.9 & Eruptive & -99.9 \\
NV247 & 17:46:04.91 & -28:45:21.19 & 0.206593 & 0.007496 & 17.79 & 13.20 & -99.9 & 9.24 & 8.8 & 8.42 & -99.9 & 11.67 & 0.83 & 1563 & SR & 1 \\
NV248 & 17:46:05.07 & -28:47:42.50 & 0.173371 & -0.01341 & -99.9 & 17.90 & 13.44 & 12.44 & 10.8 & 10.54 & -99.9 & 13.21 & 0.56 & -99.9 & IRR & -99.9 \\
NV249 & 17:46:05.15 & -28:44:18.41 & 0.221937 & 0.015828 & -99.9 & 15.21 & 12.18 & 10.79 & 10.23 & 9.48 & -99.9 & 12.15 & 0.33 & 1092 & SR & -99.9 \\
NV250 & 17:46:05.24 & -28:47:37.36 & 0.174925 & -0.01322 & -99.9 & -99.9 & 15.49 & 12.24 & 11.61 & -99.9 & -99.9 & 14.92 & 1.0 & 1291 & SR & -99.9 \\
NV251 & 17:46:05.23 & -28:49:35.75 & 0.146809 & -0.03028 & -99.9 & -99.9 & 14.59 & -99.9 & -99.9 & -99.9 & -99.9 & 13.94 & 1.23 & -99.9 & RCB? & -99.9 \\
NV252 & 17:46:05.32 & -28:49:43.71 & 0.145096 & -0.03172 & -99.9 & 15.45 & 12.28 & 10.62 & 10.07 & 9.74 & -99.9 & 12.22 & 0.27 & 1593 & SR & -99.9 \\
NV253 & 17:46:05.58 & -28:55:53.16 & 0.057937 & -0.08590 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & 14.97 & 0.93 & -99.9 & IRR & -99.9 \\
NV254 & 17:46:05.80 & -28:50:46.25 & 0.131175 & -0.04226 & -99.9 & -99.9 & 14.33 & -99.9 & -99.9 & -99.9 & -99.9 & 14.23 & 0.95 & -99.9 & IRR & -99.9 \\
NV255 & 17:46:06.03 & -28:54:23.79 & 0.079993 & -0.07439 & -99.9 & 15.68 & 11.61 & -99.9 & 9.19 & 8.9 & -99.9 & 11.76 & 0.34 & -99.9 & IRR & -99.9 \\
NV256 & 17:46:06.21 & -28:43:44.11 & 0.232092 & 0.017472 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & 13.4 & 0.96 & 1614 & SR & -99.9 \\
NV257 & 17:46:06.28 & -28:53:06.82 & 0.098730 & -0.06405 & -99.9 & -99.9 & 15.31 & -99.9 & -99.9 & -99.9 & -99.9 & 15.75 & 1.25 & -99.9 & Fader & -99.9 \\
NV258 & 17:46:06.30 & -28:52:46.38 & 0.103627 & -0.06118 & -99.9 & 16.95 & 13.51 & -99.9 & 11.55 & -99.9 & -99.9 & 13.8 & 0.91 & -99.9 & IRR & -99.9 \\
NV259 & 17:46:06.48 & -28:49:24.71 & 0.151800 & -0.03258 & -99.9 & 14.69 & 11.61 & 10.16 & 9.54 & 8.64 & -99.9 & 11.68 & 0.38 & -99.9 & IRR & -99.9 \\
NV260 & 17:46:06.78 & -28:44:03.84 & 0.228501 & 0.012829 & -99.9 & 16.25 & 12.78 & 10.76 & 10.09 & 9.26 & -99.9 & 12.7 & 0.5 & -99.9 & IRR & -99.9 \\
NV261 & 17:46:07.16 & -28:55:52.87 & 0.061011 & -0.09079 & -99.9 & 17.89 & 14.02 & 9.63 & 8.54 & 7.61 & 7.35 & 14.9 & 1.62 & -99.9 & IRR & 1 \\
NV262 & 17:46:07.27 & -28:46:00.60 & 0.201725 & -0.00555 & -99.9 & 16.24 & 13.38 & 12.04 & 11.51 & -99.9 & -99.9 & 13.37 & 0.96 & -99.9 & LPV & -99.9 \\
NV263 & 17:46:07.45 & -28:48:16.27 & 0.169888 & -0.02573 & -99.9 & 15.77 & 13.52 & -99.9 & -99.9 & -99.9 & -99.9 & 13.62 & 0.64 & -99.9 & STV & -99.9 \\
NV264 & 17:46:07.65 & -28:47:06.91 & 0.186711 & -0.01631 & -99.9 & 16.08 & 12.58 & -99.9 & -99.9 & -99.9 & -99.9 & 12.76 & 0.86 & -99.9 & IRR & -99.9 \\
NV265 & 17:46:07.67 & -28:49:23.22 & 0.154411 & -0.03607 & 19.20 & 15.54 & 12.25 & 10.29 & 9.08 & 8.45 & -99.9 & 12.23 & 0.5 & 138 & SR & -99.9 \\
NV266 & 17:46:07.69 & -28:47:30.87 & 0.181119 & -0.01992 & -99.9 & 16.85 & 13.94 & -99.9 & -99.9 & -99.9 & -99.9 & 14.03 & 0.67 & -99.9 & LPV & -99.9 \\
NV267 & 17:46:07.69 & -28:53:21.34 & 0.097971 & -0.07056 & 18.73 & 14.72 & 11.73 & 9.82 & 9.22 & 8.78 & 8.97 & 11.91 & 0.32 & -99.9 & IRR & -99.9 \\
NV268 & 17:46:07.83 & -28:46:16.97 & 0.198901 & -0.00966 & 18.68 & 14.50 & 12.14 & 10.7 & 10.53 & 10.35 & -99.9 & 12.17 & 0.27 & -99.9 & IRR & 1 \\
NV269 & 17:46:08.21 & -28:53:36.72 & 0.095306 & -0.07440 & -99.9 & 16.43 & 12.71 & -99.9 & -99.9 & -99.9 & -99.9 & 12.85 & 0.93 & 893 & SR & -99.9 \\
NV270 & 17:46:08.28 & -28:48:05.07 & 0.174110 & -0.02668 & -99.9 & 14.70 & 11.61 & 10.23 & 9.68 & 9.27 & -99.9 & 11.54 & 0.35 & -99.9 & IRR & 1 \\
NV271 & 17:46:08.46 & -28:54:07.01 & 0.088585 & -0.07954 & -99.9 & 15.87 & -99.9 & 11.9 & 11.44 & 11.18 & -99.9 & 13.19 & 0.49 & -99.9 & IRR & -99.9 \\
NV272 & 17:46:08.49 & -28:44:37.24 & 0.223817 & 0.002687 & -99.9 & 17.02 & 13.29 & 11.13 & 10.53 & 10.02 & -99.9 & 13.4 & 0.68 & 774 & SR & -99.9 \\
NV273 & 17:46:08.57 & -28:49:11.07 & 0.159017 & -0.03715 & -99.9 & -99.9 & 14.66 & -99.9 & -99.9 & -99.9 & -99.9 & 14.85 & 1.06 & -99.9 & LPV & -99.9 \\
NV274 & 17:46:08.78 & -28:44:37.68 & 0.224263 & 0.001718 & -99.9 & 16.47 & 13.01 & 10.74 & 10.22 & 9.79 & -99.9 & 13.04 & 0.37 & -99.9 & IRR & -99.9 \\
NV275 & 17:46:08.98 & -28:53:53.51 & 0.092771 & -0.07920 & -99.9 & -99.9 & 13.89 & -99.9 & 10.63 & 9.99 & 9.63 & 12.45 & 0.55 & -99.9 & IRR & -99.9 \\
NV276 & 17:46:09.04 & -28:52:15.87 & 0.116049 & -0.06528 & -99.9 & -99.9 & 14.76 & -99.9 & 12.09 & -99.9 & -99.9 & 14.67 & 1.02 & -99.9 & IRR & -99.9 \\
NV277 & 17:46:09.18 & -28:47:59.33 & 0.177184 & -0.02866 & -99.9 & 16.40 & 12.89 & 11.24 & 10.47 & 9.28 & -99.9 & 13.23 & 0.56 & -99.9 & IRR & -99.9 \\
NV278 & 17:46:09.29 & -28:47:23.30 & 0.185936 & -0.02380 & -99.9 & -99.9 & 13.39 & 12.44 & 10.79 & 10.16 & -99.9 & 13.27 & 0.6 & 443 & SR & 1 \\
NV279 & 17:46:09.35 & -28:45:45.10 & 0.209358 & -0.00981 & -99.9 & -99.9 & 14.61 & 12.3 & 12.01 & -99.9 & -99.9 & 14.46 & 1.12 & -99.9 & LPV & -99.9 \\
NV280 & 17:46:09.42 & -28:47:52.68 & 0.179225 & -0.02846 & -99.9 & 15.67 & 12.44 & 12.0 & 10.75 & -99.9 & -99.9 & 12.73 & 1.32 & 1220 & SR & 1 \\
NV281 & 17:46:09.44 & -28:46:07.09 & 0.204320 & -0.01328 & -99.9 & -99.9 & 14.30 & -99.9 & -99.9 & 9.29 & 9.17 & 14.29 & 0.8 & -99.9 & IRR & -99.9 \\
NV282 & 17:46:09.43 & -28:53:13.25 & 0.103186 & -0.07480 & -99.9 & 16.26 & 13.01 & 11.79 & -99.9 & -99.9 & -99.9 & 13.34 & 0.96 & -99.9 & LPV & -99.9 \\
NV283 & 17:46:09.57 & -28:45:19.09 & 0.215945 & -0.00674 & 19.21 & 14.43 & 11.92 & -99.9 & 9.43 & -99.9 & -99.9 & 12.04 & 0.34 & -99.9 & IRR & -99.9 \\
NV284 & 17:46:09.59 & -28:44:54.17 & 0.221901 & -0.00321 & -99.9 & 16.00 & 12.40 & 10.4 & 9.76 & 9.46 & -99.9 & 12.42 & 0.29 & 1576 & SR & 1 \\
NV285 & 17:46:09.61 & -28:47:46.99 & 0.180932 & -0.02823 & -99.9 & 15.11 & 11.60 & 9.7 & 8.97 & 8.53 & -99.9 & 11.58 & 0.6 & -99.9 & IRR & -99.9 \\
NV286 & 17:46:09.66 & -28:54:49.59 & 0.080759 & -0.08943 & -99.9 & 17.58 & 14.40 & -99.9 & -99.9 & -99.9 & -99.9 & 15.23 & 1.38 & -99.9 & LPV & -99.9 \\
NV287 & 17:46:09.83 & -28:44:45.95 & 0.224305 & -0.00277 & -99.9 & 15.78 & 12.06 & 10.14 & 9.28 & 8.8 & 8.23 & 11.77 & 0.49 & -99.9 & IRR & 1 \\
NV288 & 17:46:09.99 & -28:51:49.23 & 0.124175 & -0.06440 & -99.9 & 15.34 & 12.73 & 11.09 & 10.57 & 10.4 & -99.9 & 12.81 & 0.57 & 941 & SR & -99.9 \\
NV289 & 17:46:10.21 & -28:45:15.94 & 0.217902 & -0.00827 & -99.9 & 15.81 & 12.33 & -99.9 & 9.58 & 9.09 & 8.75 & 12.31 & 0.29 & -99.9 & IRR & -99.9 \\
NV290 & 17:46:10.21 & -28:48:01.20 & 0.178697 & -0.03215 & -99.9 & -99.9 & 14.82 & -99.9 & -99.9 & -99.9 & -99.9 & 15.21 & 1.89 & -99.9 & Dipper & -99.9 \\
NV291 & 17:46:10.26 & -28:44:47.46 & 0.224770 & -0.00433 & -99.9 & 18.09 & 14.01 & -99.9 & -99.9 & -99.9 & -99.9 & 13.72 & 0.65 & -99.9 & IRR & -99.9 \\
NV292 & 17:46:10.38 & -28:45:17.43 & 0.217872 & -0.00901 & -99.9 & 15.02 & 11.97 & 10.1 & -99.9 & 9.47 & -99.9 & 12.31 & 0.64 & -99.9 & IRR & -99.9 \\
NV293 & 17:46:10.53 & -28:48:01.79 & 0.179166 & -0.03323 & -99.9 & -99.9 & 14.95 & -99.9 & 11.36 & 10.68 & -99.9 & 15.12 & 1.11 & 1097 & LTV & -99.9 \\
NV294 & 17:46:10.61 & -28:50:59.40 & 0.137186 & -0.05915 & -99.9 & -99.9 & 13.48 & -99.9 & -99.9 & -99.9 & 10.24 & 13.38 & 0.55 & -99.9 & IRR & -99.9 \\
NV295 & 17:46:10.66 & -28:51:50.84 & 0.125073 & -0.06673 & -99.9 & -99.9 & 12.98 & 8.98 & 7.04 & 6.05 & 5.78 & 12.68 & 2.27 & 641 & Mira & 1 \\
NV296 & 17:46:10.76 & -28:52:44.75 & 0.112469 & -0.07483 & -99.9 & 17.44 & 12.93 & 11.76 & -99.9 & -99.9 & -99.9 & 12.36 & 0.78 & -99.9 & IRR & -99.9 \\
NV297 & 17:46:10.77 & -28:45:07.74 & 0.220928 & -0.00885 & -99.9 & -99.9 & 14.31 & -99.9 & -99.9 & -99.9 & -99.9 & 13.82 & 0.94 & -99.9 & IRR & -99.9 \\
NV298 & 17:46:10.97 & -28:52:04.79 & 0.122341 & -0.06970 & -99.9 & -99.9 & 13.13 & 11.72 & 10.98 & 10.39 & -99.9 & 13.38 & 0.58 & -99.9 & IRR & -99.9 \\
NV299 & 17:46:11.37 & -28:53:21.23 & 0.104975 & -0.08200 & -99.9 & 17.28 & 14.05 & -99.9 & -99.9 & -99.9 & -99.9 & 13.81 & 0.84 & -99.9 & IRR & -99.9 \\
NV300 & 17:46:11.45 & -28:45:35.00 & 0.215738 & -0.01489 & 18.26 & -99.9 & 12.38 & 11.49 & 10.8 & 10.4 & -99.9 & 12.3 & 0.29 & 1116 & SR & 1 \\
NV301 & 17:46:11.61 & -28:53:00.61 & 0.110325 & -0.07978 & -99.9 & -99.9 & 13.44 & -99.9 & 10.29 & -99.9 & -99.9 & 13.36 & 0.81 & 727 & SR & -99.9 \\
NV302 & 17:46:11.86 & -28:46:00.85 & 0.210380 & -0.01990 & -99.9 & 17.42 & 14.23 & 12.49 & 11.64 & -99.9 & -99.9 & 15.11 & 2.0 & -99.9 & RCB? & -99.9 \\
NV303 & 17:46:12.04 & -28:45:30.87 & 0.217834 & -0.01613 & -99.9 & -99.9 & 14.33 & 11.53 & 9.52 & 8.77 & -99.9 & 15.36 & 1.42 & -99.9 & Fader & -99.9 \\
NV304 & 17:46:12.06 & -28:49:49.00 & 0.156629 & -0.05348 & -99.9 & 16.88 & 14.83 & -99.9 & -99.9 & -99.9 & -99.9 & 14.93 & 0.83 & -99.9 & Dipper & -99.9 \\
NV305 & 17:46:12.16 & -28:45:21.08 & 0.220394 & -0.01511 & -99.9 & 16.75 & 13.30 & 11.86 & 11.02 & -99.9 & -99.9 & 13.18 & 0.38 & 1437 & SR & -99.9 \\
NV306 & 17:46:12.42 & -28:45:02.38 & 0.225319 & -0.01321 & -99.9 & -99.9 & 15.82 & -99.9 & -99.9 & -99.9 & -99.9 & 15.14 & 1.21 & -99.9 & Eruptive & -99.9 \\
NV307 & 17:46:12.52 & -28:48:52.45 & 0.170934 & -0.04677 & 17.31 & 14.11 & 12.23 & -99.9 & -99.9 & -99.9 & -99.9 & 12.18 & 0.39 & 1.6484 & EB & 2 \\
NV308 & 17:46:12.54 & -28:49:57.05 & 0.155643 & -0.05616 & 19.07 & 14.10 & 11.61 & 10.39 & 10.07 & 9.67 & -99.9 & 11.8 & 0.38 & -99.9 & IRR & -99.9 \\
NV309 & 17:46:12.55 & -28:44:55.40 & 0.227229 & -0.01262 & -99.9 & 16.78 & 12.87 & 11.37 & 10.38 & -99.9 & -99.9 & 12.76 & 0.38 & -99.9 & IRR & -99.9 \\
NV310 & 17:46:12.86 & -28:46:09.09 & 0.210329 & -0.02422 & -99.9 & 18.34 & 13.96 & 13.66 & 11.5 & -99.9 & -99.9 & 14.26 & 1.02 & -99.9 & IRR & -99.9 \\
NV311 & 17:46:12.94 & -28:47:16.56 & 0.194470 & -0.03421 & 17.17 & 14.83 & 13.34 & 12.61 & 12.16 & -99.9 & -99.9 & 13.34 & 0.59 & -99.9 & IRR & 1 \\
NV312 & 17:46:13.28 & -28:47:21.18 & 0.194029 & -0.03595 & 19.13 & 14.12 & 11.52 & 10.3 & -99.9 & -99.9 & -99.9 & 11.65 & 0.3 & -99.9 & IRR & -99.9 \\
NV313 & 17:46:13.32 & -28:44:54.40 & 0.228922 & -0.01486 & -99.9 & -99.9 & 14.29 & 12.66 & 12.02 & -99.9 & -99.9 & 14.16 & 1.21 & -99.9 & IRR & -99.9 \\
NV314 & 17:46:13.44 & -28:51:49.33 & 0.130699 & -0.07517 & -99.9 & 16.38 & 12.31 & -99.9 & 10.43 & 9.87 & -99.9 & 12.32 & 0.66 & 1546 & SR & -99.9 \\
NV315 & 17:46:13.50 & -28:52:52.30 & 0.115881 & -0.08446 & -99.9 & 16.11 & 12.11 & 11.16 & 9.57 & 9.15 & -99.9 & 12.18 & 0.8 & 181 & Mira & 1 \\
NV316 & 17:46:13.65 & -28:47:23.81 & 0.194096 & -0.03747 & -99.9 & 17.68 & 13.30 & -99.9 & -99.9 & -99.9 & 6.6 & 12.95 & 0.51 & 1532 & SR & -99.9 \\
NV317 & 17:46:13.71 & -28:47:14.47 & 0.196426 & -0.03631 & -99.9 & 15.27 & 12.68 & 11.55 & 11.06 & -99.9 & -99.9 & 12.77 & 0.45 & -99.9 & IRR & -99.9 \\
NV318 & 17:46:13.81 & -28:51:15.95 & 0.139326 & -0.07151 & -99.9 & 14.15 & 11.58 & 10.36 & 10.1 & 9.64 & 9.93 & 11.56 & 0.34 & -99.9 & IRR & -99.9 \\
NV319 & 17:46:13.83 & -28:44:56.69 & 0.229354 & -0.01679 & -99.9 & 14.77 & -99.9 & 9.82 & 9.47 & 8.88 & -99.9 & 11.96 & 0.39 & 428 & SR & -99.9 \\
NV320 & 17:46:13.84 & -28:47:50.39 & 0.188163 & -0.04192 & 19.01 & 15.05 & 12.40 & -99.9 & -99.9 & -99.9 & -99.9 & 12.45 & 0.29 & 1254 & SR & -99.9 \\
NV321 & 17:46:14.19 & -28:46:27.45 & 0.208498 & -0.03102 & -99.9 & 15.09 & 12.90 & 11.02 & -99.9 & 9.92 & -99.9 & 12.85 & 0.51 & -99.9 & IRR & -99.9 \\
NV322 & 17:46:14.36 & -28:46:09.51 & 0.213075 & -0.02896 & -99.9 & -99.9 & 15.02 & -99.9 & -99.9 & -99.9 & -99.9 & 15.35 & 1.5 & -99.9 & Dipper & -99.9 \\
NV323 & 17:46:14.50 & -28:50:30.64 & 0.151392 & -0.06712 & -99.9 & 16.62 & 13.90 & -99.9 & -99.9 & -99.9 & -99.9 & 14.07 & 0.73 & -99.9 & LPV & -99.9 \\
NV324 & 17:46:14.80 & -28:52:55.82 & 0.117512 & -0.08903 & -99.9 & -99.9 & 14.48 & -99.9 & -99.9 & -99.9 & -99.9 & 14.71 & 1.22 & -99.9 & IRR & -99.9 \\
NV325 & 17:46:14.86 & -28:45:53.42 & 0.217860 & -0.02822 & -99.9 & 16.31 & 12.68 & 11.1 & 10.23 & 9.6 & -99.9 & 12.62 & 0.85 & -99.9 & IRR & -99.9 \\
NV326 & 17:46:14.95 & -28:46:47.84 & 0.205102 & -0.03633 & -99.9 & 15.75 & 12.23 & 10.88 & 9.48 & 9.47 & -99.9 & 12.27 & 0.61 & -99.9 & IRR & -99.9 \\
NV327 & 17:46:14.98 & -28:51:52.90 & 0.132770 & -0.08048 & -99.9 & 17.20 & 15.45 & -99.9 & -99.9 & -99.9 & -99.9 & 15.34 & 1.48 & -99.9 & Eruptive & -99.9 \\
NV328 & 17:46:15.25 & -28:51:21.60 & 0.140726 & -0.07683 & -99.9 & 16.25 & 12.99 & -99.9 & 11.13 & 10.78 & -99.9 & 12.84 & 0.45 & -99.9 & IRR & -99.9 \\
NV329 & 17:46:15.29 & -28:51:01.69 & 0.145523 & -0.07407 & -99.9 & -99.9 & 15.11 & -99.9 & -99.9 & -99.9 & -99.9 & 15.33 & 1.54 & -99.9 & Dipper & -99.9 \\
NV330 & 17:46:15.47 & -28:47:00.89 & 0.203004 & -0.03986 & -99.9 & 16.92 & 11.90 & -99.9 & 8.81 & 8.23 & 8.29 & 11.63 & 0.48 & 322 & SR & 1 \\
NV331 & 17:46:15.95 & -28:45:31.76 & 0.225066 & -0.02849 & -99.9 & 17.21 & 13.24 & 11.03 & 10.07 & 9.84 & -99.9 & 13.44 & 1.03 & 823 & SR & -99.9 \\
NV332 & 17:46:16.00 & -28:45:01.88 & 0.232238 & -0.02431 & -99.9 & -99.9 & -99.9 & 12.58 & 12.02 & -99.9 & -99.9 & 13.8 & 0.7 & -99.9 & IRR & -99.9 \\
NV333 & 17:46:16.59 & -28:45:25.51 & 0.227755 & -0.02956 & -99.9 & -99.9 & 14.99 & 12.88 & 11.81 & -99.9 & -99.9 & 15.14 & 1.13 & 523 & SR & -99.9 \\
NV334 & 17:46:16.89 & -28:46:42.34 & 0.210096 & -0.04160 & 17.78 & 16.27 & 13.78 & 13.07 & 11.89 & -99.9 & -99.9 & 14.02 & 0.74 & -99.9 & LPV & -99.9 \\
NV335 & 17:46:17.28 & -28:46:53.37 & 0.208215 & -0.04440 & -99.9 & 16.20 & 12.23 & 11.04 & 9.92 & 8.78 & -99.9 & 12.17 & 0.55 & 436 & SR & 1 \\
NV336 & 17:46:17.94 & -28:45:35.11 & 0.228035 & -0.03515 & -99.9 & 16.79 & 13.65 & -99.9 & 11.52 & -99.9 & -99.9 & 13.72 & 0.77 & -99.9 & IRR & -99.9 \\
NV337 & 17:46:18.24 & -28:45:24.07 & 0.231237 & -0.03452 & -99.9 & -99.9 & -99.9 & 11.21 & 10.33 & 10.2 & -99.9 & 13.12 & 1.27 & -99.9 & RCB? & -99.9 \\
NV338 & 17:46:18.62 & -28:51:32.37 & 0.144562 & -0.08889 & -99.9 & 17.0 & 13.07 & 11.25 & 10.56 & 10.14 & 10.1 & 13.08 & 0.71 & 294 & SR & -99.9 \\
NV339 & 17:46:19.46 & -28:49:25.61 & 0.176221 & -0.07318 & -99.9 & -99.9 & 14.92 & -99.9 & 11.34 & -99.9 & -99.9 & 15.26 & 1.47 & -99.9 & Dipper & -99.9 \\
NV340 & 17:46:19.48 & -28:47:40.72 & 0.201167 & -0.05812 & -99.9 & -99.9 & 13.60 & 12.34 & 11.9 & -99.9 & -99.9 & 13.76 & 0.67 & -99.9 & IRR & -99.9 \\
NV341 & 17:46:20.37 & -28:47:43.33 & 0.202234 & -0.06127 & -99.9 & 16.39 & 13.05 & -99.9 & 11.38 & -99.9 & -99.9 & 13.28 & 1.0 & -99.9 & IRR & -99.9 \\
NV342 & 17:46:20.96 & -28:46:02.50 & 0.227285 & -0.04856 & -99.9 & 17.99 & -99.9 & -99.9 & -99.9 & -99.9 & -99.9 & 14.37 & 0.98 & -99.9 & LPV & -99.9 \\
NV343 & 17:46:21.22 & -28:49:10.80 & 0.183083 & -0.07654 & -99.9 & 16.46 & 13.54 & -99.9 & -99.9 & -99.9 & -99.9 & 13.2 & 0.56 & -99.9 & IRR & -99.9 \\
NV344 & 17:46:21.31 & -28:46:27.13 & 0.222099 & -0.05320 & -99.9 & 17.36 & 15.10 & -99.9 & -99.9 & -99.9 & -99.9 & 15.03 & 1.42 & -99.9 & Dipper & -99.9 \\
NV345 & 17:46:21.83 & -28:50:31.03 & 0.165199 & -0.09003 & -99.9 & 18.12 & 15.57 & -99.9 & -99.9 & -99.9 & -99.9 & 14.96 & 1.8 & -99.9 & Eruptive/EXor & -99.9 \\
NV346 & 17:46:22.44 & -28:47:19.54 & 0.211800 & -0.06428 & -99.9 & 15.05 & 11.88 & 10.33 & 9.91 & 9.2 & -99.9 & 11.93 & 0.27 & 447 & SR & -99.9 \\
NV347 & 17:46:23.04 & -28:50:01.99 & 0.174383 & -0.08960 & 18.51 & 13.77 & -99.9 & 10.44 & 9.75 & 9.71 & 10.05 & 11.37 & 0.3 & -99.9 & IRR & 1 \\
NV348 & 17:46:23.50 & -28:47:17.21 & 0.214376 & -0.06727 & -99.9 & 15.37 & 12.77 & 11.13 & 10.51 & 10.12 & -99.9 & 12.89 & 0.47 & -99.9 & IRR & -99.9 \\
NV349 & 17:46:24.57 & -28:47:46.22 & 0.209512 & -0.07478 & -99.9 & 15.05 & 12.09 & 10.48 & 9.97 & 9.53 & -99.9 & 12.17 & 0.47 & -99.9 & IRR & -99.9 \\
NV350 & 17:46:27.35 & -28:46:55.41 & 0.226850 & -0.07613 & 18.42 & 14.53 & -99.9 & 10.23 & 9.81 & 9.23 & -99.9 & 11.63 & 0.26 & -99.9 & IRR & -99.9 \\
NV351 & 17:46:28.63 & -28:48:01.75 & 0.213524 & -0.08968 & -99.9 & 17.21 & 15.32 & -99.9 & -99.9 & -99.9 & -99.9 & 15.13 & 1.94 & -99.9 & Microlensing & -99.9 \\
NV352 & 17:46:29.63 & -28:47:51.24 & 0.217914 & -0.09128 & -99.9 & -99.9 & 14.73 & -99.9 & 11.89 & -99.9 & -99.9 & 14.83 & 0.96 & -99.9 & IRR & -99.9 \\
NV353 & 17:46:29.84 & -28:47:14.00 & 0.227165 & -0.08659 & -99.9 & 18.06 & 14.16 & 11.19 & 10.38 & 9.89 & -99.9 & 14.22 & 0.93 & -99.9 & IRR & -99.9 \\
\hline
	\multicolumn{13}{l}{$^a$ {\bf References.} (1) \citetalias{mkn09}; (2) \citetalias{mfk13}; (3) \citet{woo98}.}
    \end{tabular}
\end{table}
\end{landscape}
